A note on the Burris-Willard conjecture

Based on results by Dani\v{l}\v{c}enko, in 1987 Burris and Willard have conjectured that on any $k$-element domain where $k\geq 3$ it is possible to bicentrically generate every centraliser clone from its $k$-ary part. Later, for every $k\geq 3$, Snow constructed algebras with a $k$-element carrier set where the minimum arity of the clone of term operations from which the bicentraliser can be generated is at least $(k-1)^2$, which is larger than $k$ for $k\geq 3$. We prove that Snow's examples do not violate the Burris-Willard conjecture nor invalidate the results by Dani\v{l}\v{c}enko on which the latter is based. We also complement our results with some computational evidence for $k=3$, obtained by an algorithm to compute a primitive positive definition for a relation in a finitely generated relational clone over a finite set.

==> hyphexcept.tex <==
%1 vim: set ft=tex:
%2 Use ./sorthyph.sh to bring this file in alphabetical order.
%3 This is essentially the command `sort -d -f'.
\hyphenation{an-aly-ses}
\hyphenation{an-aly-sis}
\hyphenation{as-so-cia-tive}
\hyphenation{as-so-cia-tiv-ity}
\hyphenation{auto-morph-ic}% (2!)
%\hyphenation{auto-morph-ism}% okay
%\hyphenation{auto-morph-isms}% okay
\hyphenation{au-tono-mous}
\hyphenation{au-tono-mous-ly}% (2!)
\hyphenation{be-tween}
\hyphenation{Bool-ean}
\hyphenation{bound-ed}% (2!)
\hyphenation{Car-te-sian}
%\hyphenation{cat-e-go-ries} %AE??
%\hyphenation{cat-egor-ies}% okay
\hyphenation{com-mu-ta-tive}
\hyphenation{com-mu-ta-tiv-ity}
\hyphenation{con-se-quence}
\hyphenation{con-se-quences}
\hyphenation{con-se-quent-ly}% (2!)
\hyphenation{Con-se-quent-ly}% (2!)
\hyphenation{co-ord-in-ate}
\hyphenation{def-in-ition}
\hyphenation{Def-in-ition}
\hyphenation{def-in-itions}
\hyphenation{Def-in-itions}
\hyphenation{de-ter-mine}
\hyphenation{de-ter-mined}
\hyphenation{de-ter-mined-ly}% (2!)
\hyphenation{de-ter-min-ing}
\hyphenation{endo-morph-ic}% (2!)
\hyphenation{endo-morph-ism}
\hyphenation{endo-morph-isms}
\hyphenation{equiva-lence}
\hyphenation{equiva-lences}
\hyphenation{equiva-lent}
\hyphenation{equiva-lent-ly}% (2!)
\hyphenation{homeo-morph-ic-al-ly}% (!2)
\hyphenation{Homeo-morph-ic-al-ly}% (!2)
\hyphenation{homeo-morph-ic-ity}%
\hyphenation{Homeo-morph-ic-ity}%
%\hyphenation{homeo-morph-ism}% okay
%\hyphenation{homeo-morph-isms}% okay
\hyphenation{idem-po-tents}
\hyphenation{idem-po-tent}% see po-tent
\hyphenation{iden-ti-cal}
\hyphenation{im-pli-ca-tion}
\hyphenation{Im-pli-ca-tion}
\hyphenation{im-pli-ca-tions}
\hyphenation{Im-pli-ca-tions}
\hyphenation{ir-re-du-ci-bil-ity}
%%\hyphenation{ir-re-duc-ibil-i-ty}% AE?
%%\hyphenation{ir-re-duc-ible}% AE?
%\hyphenation{ir-re-du-cible}% okay
%\hyphenation{ir-re-du-cibly}% okay
\hyphenation{iso-morph-ic} % last hyphen probably not recognised due to
%\hyphenation{iso-morph-ism}% okay
%\hyphenation{iso-morph-isms}% okay
\hyphenation{lem-ma}% (2!) % BE: not at all
\hyphenation{Lem-ma}% (2!) BE: not at all
\hyphenation{more-over}
\hyphenation{More-over}
\hyphenation{neigh-bour-hood}
\hyphenation{neigh-bour-hoods}
\hyphenation{non-au-tono-mous}
\hyphenation{poly-morph-ic}% (!2)
%\hyphenation{poly-morph-ism}% okay
%\hyphenation{poly-morph-isms}% okay
\hyphenation{posi-tive-ly}% (!2)
\hyphenation{prod-uct}
\hyphenation{prod-ucts}
\hyphenation{re-la-tion-al}% (2!)
\hyphenation{re-la-tion-al-ly}% (2!)
\hyphenation{semi-group}
\hyphenation{semi-groups}
\hyphenation{semi-lat-tice}
\hyphenation{semi-lat-tices}
\hyphenation{strength-en}% (2!)
\hyphenation{strength-ened}
\hyphenation{tauto-logic-al}% (2!)
\hyphenation{tauto-logic-al-ly}% (2!)
\hyphenation{tau-tolo-gies}
\hyphenation{tau-tolo-gous}
\hyphenation{tau-tol-ogy}
\hyphenation{topo-logic-al}% (2!)
\hyphenation{topo-logic-al-ly}% (2!)
\hyphenation{top-olo-gies}
\hyphenation{Top-olo-gies}
\hyphenation{top-ology}
\hyphenation{Top-ology}
\hyphenation{when-ever}

